Shape Distributions of Nonlinear Dynamical Systems for Video-based Inference

This paper presents a shape-theoretic framework for dynamical analysis of nonlinear dynamical systems which appear frequently in several video-based inference tasks. Traditional approaches to dynamical modeling have included linear and nonlinear methods with their respective drawbacks. A novel approach we propose is the use of descriptors of the shape of the dynamical attractor as a feature representation of nature of dynamics. The proposed framework has two main advantages over traditional approaches: a) representation of the dynamical system is derived directly from the observational data, without any inherent assumptions, and b) the proposed features show stability under different time-series lengths where traditional dynamical invariants fail. We illustrate our idea using nonlinear dynamical models such as Lorenz and Rossler systems, where our feature representations (shape distribution) support our hypothesis that the local shape of the reconstructed phase space can be used as a discriminative feature. Our experimental analyses on these models also indicate that the proposed framework show stability for different time-series lengths, which is useful when the available number of samples are small/variable. The specific applications of interest in this paper are: 1) activity recognition using motion capture and RGBD sensors, 2) activity quality assessment for applications in stroke rehabilitation, and 3) dynamical scene classification. We provide experimental validation through action and gesture recognition experiments on motion capture and Kinect datasets. In all these scenarios, we show experimental evidence of the favorable properties of the proposed representation.

==> README <==
January 10, 2007

Please note that you may choose to use either double column or single column
formatting. You may wish to use single column formatting when submitting your
paper for review, as it leaves more space for reviewer remarks. The double column format 
is ideal when submitting your final publication materials. The IEEE CS formats articles
in two columns, with 9.5pt Palatino font, and a page size of 7.875 X 10.75. 

June 6, 2006

Added an option to switch between peer review and final submission formats 
into bare_jrnl.tex. 


August 13, 2002

This IEEEtran.cls is the official LaTeX class for authors of the
Institute of Electrical and Electronics Engineers (IEEE) transactions
journals and conferences. In addition to being carried on IEEE's site,
IEEEtran.cls may be found at:

http://www.ctan.org/tex-archive/macros/latex/contrib/supported/IEEEtran/

The CTAN site may have additional files related to non-IEEE uses of this
tool.

As of version 1.6, IEEEtran.cls now provides support for conferences and
A4 paper. Users of previous versions should no longer manually alter margins,
paper sizes, page styles, etc. Also, please note that \author is used
slightly differently from that of V1.5, especially for conferences.
\pubid (if used) must now be placed before \maketitle. \cite is now robust
and can be used within captions without a proceeding \protect.

As with previous versions, The itemize, enumerate, and description lists as
well as \appendix(ces) have enhanced controls and work slightly differently
than is done in traditional LaTeX.

Extensive formal documentation is now available. Enjoy! ;) The appendices
of the user manual contain important information on avoiding commonly
made mistakes, compatibility issues and installation instructions.


Best wishes for all your publication endeavors,

Michael Shell
mshell@ece.gatech.edu



********************* Files **********************

README               - This file.

IEEEtran.cls         - The LaTeX class file.

IEEEtran_HOWTO.pdf   - The user manual.

bare_jrnl.tex        - A "bare bones" starter file for journal papers.




**********************************************************************
 Legal Notice:
 This code and advice is offered as-is without any warranty either
 expressed or implied; without even the implied warranty of
 MERCHANTABILITY or FITNESS FOR A PARTICULAR PURPOSE!
 User assumes all risk.
 In no event shall IEEE or any contributor to this code
 be liable for any damages or losses, including, but not limited to,
 incidental, consequential, or any other damages, resulting from the
 use or misuse of any information contained here.
 
 All statements made here are the opinions of their respective
 authors and are not necessarily endorsed by the IEEE.

 This code/text is distributed under the Perl Artistic License 
 ( http://language.perl.com/misc/Artistic.html ) 
 and may be freely used, distributed and modified.
 Retain all contribution notices and credits.
**********************************************************************



